Aligning Graphical and Functional Causal Abstractions

Causal abstractions allow us to relate causal models on different levels of granularity. To ensure that the models agree on cause and effect, frameworks for causal abstractions define notions of consistency. Two distinct methods for causal abstraction are common in the literature: (i) graphical abstractions, such as Cluster DAGs, which relate models on a structural level, and (ii) functional abstractions, like $\alpha$-abstractions, which relate models by maps between variables and their ranges. In this paper we will align the notions of graphical and functional consistency and show an equivalence between the class of Cluster DAGs, consistent $\alpha$-abstractions with the range of abstracted variables mapped bijectively, and constructive $\tau$-abstractions. Furthermore, we extend this alignment and the expressivity of graphical abstractions by introducing Partial Cluster DAGs. Our results provide a rigorous bridge between the functional and graphical frameworks and allow for adoption and transfer of results between them.

==> Parts/Lemma-Adjancent-Confounding-Edges.tex <==
\begin{lemma}[Adjacent Confounding Edges from $\ltwo$ distributions]\label{lem:adj-conf}
   Given some $X, Y \in \vars$ of a model $\model$ such that $X \rightarrow Y$ is an adjacency, all confounding edges $X\confarrow Y$ can be identified by comparing $\ltwo$ distributions.
    \begin{proof}
        Proof is given in appendix \ref{proof-adj-conf}.
    \end{proof}
\end{lemma}

==> Parts/Lemma-Non-Adjacent-Confounding-Edges.tex <==
\begin{lemma}[Non-Adjacent Confounding Edges from $\ltwo$ distributions]\label{lem:non-adj-conf}
    Given some $X, Y \in \vars$ of a model $\model$ such that $X$ and $Y$ are not adjacent all confounding edges $X\confarrow Y$ can be identified by comparing $\ltwo$ distributions.
    \begin{proof}
        Proof is given in appendix \ref{proof-non-adj-conf}.
    \end{proof}
\end{lemma}

==> Parts/Lemma-Preservation-Directed-Paths.tex <==
\begin{lemma}[Interventional Consistency Preservers Directed Paths]\label{lem:consistency-directed-paths}
     Interventional consistency \\of prefect $\alpha$-abstractions preserve directed paths between variables: Let $\mathcal M$ be an SCM, and $\mathcal M'$ an SCM that is a perfect $\alpha$-abstraction of $\mathcal M$. If there exist a path $\mathbf C_i \rightarrow \cdots \rightarrow \mathbf C_j$ with $\mathbf C_i, \mathbf C_j \in G(\mathcal M')$ then there exist a path $V_i \rightarrow \cdots \rightarrow V_j$ with $V_i, V_j \in G(\mathcal M), \; f(V_i) = C_i, \; f(V_j)=C_j$.
     \begin{proof}
         Proof is given in appendix \ref{proof-int-conf-dir-paths}
     \end{proof}
\end{lemma}

==> Parts/Proof-Adjacent-Confounding-Edges.tex <==
\begin{customlemma}{\ref{lem:adj-conf}}[Adjacent Confounding Edges from $\ltwo$ distributions]
   Given some $X, Y \in \vars$ of a model $\model$ such that $X \rightarrow Y$ is an adjacency, all confounding edges $X\confarrow Y$ can be identified by comparing $\ltwo$ distributions.
    \begin{proof}\normalfont
        Given some $X,Y\in \vars$ of $\model$, such that $X\rightarrow Y$. we will show that the absence of a confounder $X\confarrow Y$ implies $P(Y\:|\:X,do(\mathbf Z)) = P(Y\:|\:do(X),do(\mathbf Z))$. Secondly, we show that the presence of a confounder $X\confarrow Y$ implies $P(Y\:|\:X,do(\mathbf Z))\neq P(Y\:|\:do(X),do(\mathbf Z))$.

        First, recall that any indirect path between $X$ and $Y$ can be blocked by some $\mathbf Z \in \vars \setminus\{X,Y\}$. It follows that given such a $\mathbf Z$ we have $P(Y\:|\:X,do(\mathbf Z)) = P(Y\:|\:do(X),do(\mathbf Z))$.

        Now let's consider the following diagram:
        \begin{tikzcd}
            X\arrow[r]\arrow[r, bend left, dashed, <->, "U"]& Y.
        \end{tikzcd}
        Recall that $X\confarrow Y$ is an shorthand for writing $X\leftarrow U \rightarrow Y$. Note also that an arrow $X\rightarrow Y$ implies $P(Y)\neq P(Y\:|\:X)$ and $P(X)\neq P(X\:|\:Y)$, assuming non-canceling paths. Now consider what happens when we condition on $X$ by taking $P(Y\:|\:X)$. As we have an arrow $U\rightarrow X$ we get that $P(U\:|\:X)\neq P(U)$.

        \sloppy Alternatively, if we consider $P(Y\:|\:do(X))$ we break the edge $U\rightarrow X$, so $P(U)=P(U\:|\:do(X))$. Furthermore the distributions $P(Y\:|\:X)$ and $P(Y\:|\:do(X))$ are determined by a function $f_Y(U, U_Y, X)$ with $U_Y$ an optional exogenous variable affecting $Y$. We see that given $X$ and a distribution $P(U_Y)$ the generated distributions depend only on the distribution $P(U)$, and since we have shown that $P(U\:|\:do(X))=P(U)\neq P(U\:|\:X)$ it follows that $P(Y\:|\:X)\neq P(Y\:|\:do(X))$. In case our model has more variables than $X$ and $Y$ we can block any other path with some $\mathbf Z$, as done in Lemma \ref{lem:non-adj-conf}.

        In conclusion, given two adjacent variables $X,Y$ such that $X\rightarrow Y$, there exists a confounding arrow $X\confarrow Y$ if, and only if, $P(Y\:|\:X,do(\mathbf Z))\neq P(Y\:|\:do(X),do(\mathbf Z))$.
    \end{proof}
\end{customlemma}

==> Parts/Proof-Consistency-Determines-Structure.tex <==
\begin{customthm}{\ref{thm:Consistency-Structure}}[$\ltwo$-Consistency Uniquely Determines Structure of a Model]\\
    Given a bijective $\ltwo$-consistent abstraction $\boldsymbol{\alpha}: \mathcal M\rightarrow \mathcal M'$ the structure of the graph $G'$ underlying $\model'$ is uniquely determined by the maps $\varphi:\vars \rightarrow \mathbf C$.

    \begin{proof} \normalfont
        The proof follows partially from Lem.\ref{lem:interventional-consistency-adjacency}: $\ltwo$-consistency uniquely determines causal edges of an abstraction.

        Furthermore, Lem.\ref{lem:L2-conf} shows that confounding edges are uniquely determined by $\ltwo$ distributions of a model. Recall that these lemmas rely on equalities and inequalities of $\ltwo$ distributions, and that Lem.\ref{lem:consistency-Equalities} shows that these equalities and inequalities are preserved under a bijective $\ltwo$-consistent $\alpha$-abstraction if the domain maps are bijective. It follows that the confounding edges of a bijective $\ltwo$-consistent $\alpha$-abstraction are uniquely given by $\varphi$.

        Considering that both causal edges and confounding edges are uniquely determined for a bijective $\ltwo$-consistent $\alpha$-abstraction.
    \end{proof}
\end{customthm}

==> Parts/Proof-Non-Adjacent-Confounding-Edges.tex <==
\begin{customlemma}{\ref{lem:non-adj-conf}}[Non-Adjacent Confounding Edges from $\ltwo$ distributions]
    Given some $X, Y \in \vars$ of a model $\model$ such that $X$ and $Y$ are not adjacent all confounding edges $X\confarrow Y$ can be identified by comparing $\ltwo$ distributions.
    \begin{proof}\normalfont
        For this proof we will show that given two variables $X, Y \in \vars$ of a model $\model$ with $X$ and $Y$ not adjacent there exists some $\mathbf  Z \subseteq \vars\setminus\{X,Y\}$ such that $P(Y\:|\:X, do(\mathbf Z)) = P(Y\:|\:do(\mathbf Z))$ if and only if there does not exist a confounding edge $X\confarrow Y$. First we show that non existence of a confounding edge $X \confarrow Y$ implies $P(Y\:|\:X, do(\mathbf Z)) = P(Y\:|\:do(\mathbf Z))$. After we show that $X \confarrow Y$ implies $P(Y\:|\:X, do(\mathbf Z)) \neq P(Y\:|\:do(\mathbf Z))$, completing the proof.
        
        First, assume $X$ and $Y$ do not share a confounding edge $X\confarrow Y$. Non-adjacency gives us that there exists some $\mathbf Z \subset \vars\setminus \{X,Y\}$ blocking all paths between $X$ and $Y$ that have at least one intermediate vertex in $\vars$. A path without a vertex in $\vars$ would imply $X\confarrow Y$, which by assumption do not exist. We get that there exists some $\mathbf Z \subset \vars\setminus \{X,Y\}$ st. $Y\ind X \:|\:do(\mathbf Z)$. Or, in terms of distributions: $P(Y\:|\:X, do(\mathbf Z)) = P(Y\:|\:do(\mathbf Z))$ for all non-adjacent $X,Y$ if there does not exist a confounding edge $X\confarrow Y$. 

        Secondly, we show the inverse: assume there exists a confounding edge $X\confarrow Y$. By assumption of $X\confarrow Y$ we have a path between $X$ and $Y$ that cannot be blocked by any intervention. So there cannot exist a $\mathbf Z \in \vars \setminus \{X,Y\}$ st. $Y\ind X \:|\:do(\mathbf Z)$. This is expressed in terms of distributions as $P(Y\:|\:X, do(\mathbf Z)) \neq P(Y\:|\:do(\mathbf Z))$ for all $\mathbf Z$, if we have $X\confarrow Y$.
        
        We conclude that all confounding edges between two non-adjacent variables $X$ and $Y$ can be identified using $\ltwo$ distributions.
    \end{proof}
\end{customlemma}

==> Parts/Proof-PCDAG-D-Separation.tex <==
\begin{customthm}{\ref{thm:PCDAG-D-Separation}}[D-separation is consistent in Partial Cluster DAGs]
     Let $\mathcal M'$ be a Partial Cluster DAG of a SCM $\mathcal M$ together with a clustering $\mathbf C$ of the variables $\mathbf V$ of $\mathcal M$. Let $\mathbf X,\mathbf Y,\mathbf Z \underset{disjoint}{\subseteq} \mathbf C$ be disjoint subsets of clusters of $\mathcal M'$. Let $\mathbf X', \mathbf Y', \mathbf Z'$ denote the sets of variables in $\mathbf V$ of $\mathcal M$ that make up the clusters. Then $X\ind_{\mathcal M'} Y  \:|\: Z$ if and only if $X'\ind_{\mathcal M} Y' \:|\: Z'$.
     
    \begin{proof}
        TODO: Put this in
    \end{proof}
\end{customthm}

==> Parts/Proof-PCDAG-Do-Calculus.tex <==
\begin{customthm}{\ref{thm:PCDAG-do-calculus}}[Do-calculus is consistent in Partial Cluster DAGs]
    \sloppy Let $\mathcal M'$ be a Partial Cluster DAG for a causal model $\mathcal M$ with the clustering $\mathbf C = \{\mathbf C_1 ,\dots \mathbf C_n\}$, and let $X,Y,Z,W \underset{disjoint}{\subseteq} \mathbf C$, and $G = G(\mathcal M')$ the three rules of do-calculus hold:
    \begin{center}
        $\mathbf{1.} \;\;\; P(y|\:do(X=x), z, w) = P(y|\: do(x),w)$\\
        $\text{if } (Y\ind Z|X,W)_{G_{C_{\overline{X}}}}$
    \end{center}
    \begin{center}
        $\mathbf{2.} \;\;\; P(y|\:do(X=x), do(Z=z), w) = P(y|\: do(x),z,w)$\\
        $\text{if } (Y\ind Z|X,W)_{G_{C_{\overline{X}\underline{Z}}}}$
    \end{center}
    \begin{center}
        $\mathbf{3.} \;\;\; P(y|\:do(X=x), do(Z=z), w) = P(y|\: do(x),w)$\\
        $\text{if } (Y\ind Z|X,W)_{G_{C_{\overline{XZ(W)}}}}$
    \end{center}
    
    \begin{proof}
        TODO: Put this in
    \end{proof}
\end{customthm}

==> Parts/Proof-Preservation-Directed-Paths.tex <==
\begin{customlemma}{\ref{lem:consistency-directed-paths}}[Interventional Consistency Preservers Directed Paths]
     Given a prefect $\alpha$-\\abstraction $\alpha: \mathcal M \rightarrow \mathcal M'$ from SCM $\mathcal M$ to SCM $\mathcal M'$. Let $\mathbf{V}$ be the set of endogenous variables of $\mathcal M$ and $\mathbf C$ be a clustering of $\mathbf V$. If there exist a path $V_i \rightarrow \cdots \rightarrow V_j$ with $V_i, V_j \in \mathbf V, \; f(V_i) = \mathbf C_i\in \mathbf C$ in $\mathcal M$, then there exists a path $C_i \rightarrow \cdots \rightarrow C_j$ with in $\mathcal M'$.

    \begin{proof} \normalfont
        Interventional consistency gives us $P(Y |\; do(X)) = \alpha\left[P(f^{-1}(Y)|\;do(f^{-1}(X))\right]$ for all $Y,X \subseteq G(M')$. Let $Y\in G(\mathcal M')$ be a single vertex in $G(\mathcal M')$, then we have 
        \begin{align*}
            P(Y |\;do(\emptyset)) &= \alpha\left[P(f^{-1}(Y)|\;do(\emptyset))\right],\\
            P(Y |\;do(X)) &= \alpha\left[P(f^-(Y)|\;do(f^{-1}(X))\right].
        \end{align*}
        First we note that $P(f^{-1}(Y)|\;do(f^{-1}(X)) = P(f^{-1}(Y)|\;do(\emptyset))$ implies $f^{-1}(Y) \ind f^{-1}(X)$ in $G(\mathcal M)$. That is, there exists no directed path $f^{-1}(X) \rightarrow \cdots \rightarrow f^{-1}(Y)$ in $G(\mathcal M)$. Similarly, $P(Y|\;do(X)) = P(Y|\;do(\emptyset))$, implies that there exists no directed path $Y \rightarrow \cdots \rightarrow X$ in $G(\mathcal M')$. Secondly, if follows from the equations that $P(f^{-1}(Y)|\;do(f^{-1}(X)) = P(f^{-1}(Y)|\;do(\emptyset))$ necessarily implies $P(Y|\;do(X)) = P(Y|\;do(\emptyset))$. Consequently, we conclude that the absence of a directed path $f^-(X) \rightarrow \cdots \rightarrow f^-(Y)$ in $G(\mathcal M)$ implies the absence of a directed path $X \rightarrow \cdots \rightarrow Y$ in $G(\mathcal M')$.
        
        Now we proof the other direction: Let $Y \ind X$ in $G(\mathcal M')$. We get that $P(Y|\; do(X)) = P(Y|\;do(\emptyset))$ by independence of $Y$ and $X$. Consider the case where $f^{-1}(Y) \nind f^{-1}(X)$ in $G(\mathcal M)$. We have that $$P(f^{-1}(Y)|\; do(f^{-1}(X))) \neq P(f^{-1}(Y)|\;do(\emptyset)).$$ Following the $\alpha$-abstraction, we get 
        $$P(Y|\;do(X)) \neq P(Y|\;do(\emptyset)),$$ giving rise to a contradiction. We conclude that $Y \ind X$ in $G(\mathcal M')$ implies $f^{-1}(Y) \ind f^{-1}(X)$ in $G(\mathcal M)$.
    
        Now that we have shown both sides we can conclude that given a perfect $\alpha$-abstraction $\alpha : \mathcal M \rightarrow \mathcal M'$ a directed path $X \rightarrow \dots \rightarrow Y$ is in $G(M')$ iff a directed path $f^{-1}(X) \rightarrow \dots \rightarrow f^{-1}(Y)$ is in $G(\mathcal M)$.
    \end{proof}
\end{customlemma}

==> Parts/Theorem-Consistency-Determines-Structure.tex <==
%Structure of an Abstraction is Uniquely Determined by $\ltwo$ Consistency
\begin{theorem}[$\ltwo$-Consistency Uniquely Determines the Structure of a Model]\label{thm:Consistency-Structure}
    Given a bijective $\ltwo$-consistent abstraction $\boldsymbol{\alpha}: \mathcal M\rightarrow \mathcal M'$ the structure of the graph $G'$ underlying $\model'$ is uniquely determined by the maps $\varphi:\vars \rightarrow \mathbf C$. \emph{[Proof in App. \ref{proof-l2-structure-abstraction}.]}

    %\begin{proof}
    %    Proof is given in appendix \ref{proof-l2-structure-abstraction}.
    %\end{proof}
\end{theorem}

==> Parts/Theorem-PCDAG-D-Separation.tex <==
\begin{theorem}[D-separation is consistent in Partial Cluster DAGs]\label{thm:PCDAG-D-Separation}
     Let $\mathcal M'$ be a Partial Cluster DAG of a SCM $\mathcal M$ together with a clustering $\mathbf C$ of the variables $\mathbf V$ of $\mathcal M$. Let $\clusts_\mathbf{X},\clusts_\mathbf{Y},\clusts_\mathbf{Z} \underset{disjoint}{\subseteq}\nolinebreak \clusts$ be disjoint subsets of clusters of $\mathcal M'$. Let $\mathbf X, \mathbf Y, \mathbf Z$ denote the sets of variables in $\mathbf V$ of $\mathcal M$ that make up the clusters. $\clusts_\mathbf{X}\ind_{\mathcal M'} \clusts_\mathbf{Y}  \:|\: \clusts_\mathbf{Z}$ if and only if $\mathbf{X}\ind_{\mathcal M} \mathbf{Y} \:|\: \mathbf{Z}$.

     \begin{proof}
         Proof is given in appendix \ref{proof-d-separation}.
     \end{proof}
\end{theorem}

==> Parts/Theorem-PCDAG-Do-Calculus.tex <==
\begin{theorem}[Do-calculus is consistent in Partial Cluster DAGs]\label{thm:PCDAG-do-calculus}
    Let $\mathcal M'$ be a Partial Cluster DAG for a causal model $\mathcal M$ with the clustering $\mathbf C = \{\mathbf C_1 ,\dots \mathbf C_n\}$, and let $X,Y,Z,W \underset{disjoint}{\subseteq} \mathbf C$, and $G = G(\mathcal M')$ the three rules of do-calculus hold:
    \begin{center}
        $\mathbf{1.} \;\;\; P(y|\:do(X=x), z, w) = P(y|\: do(x),w)$\\
        $\text{if } (Y\ind Z|X,W)_{G_{C_{\overline{X}}}}$
    \end{center}
    \begin{center}
        $\mathbf{2.} \;\;\; P(y|\:do(X=x), do(Z=z), w) = P(y|\: do(x),z,w)$\\
        $\text{if } (Y\ind Z|X,W)_{G_{C_{\overline{X}\underline{Z}}}}$
    \end{center}
    \begin{center}
        $\mathbf{3.} \;\;\; P(y|\:do(X=x), do(Z=z), w) = P(y|\: do(x),w)$\\
        $\text{if } (Y\ind Z|X,W)_{G_{C_{\overline{XZ(W)}}}}$
    \end{center}

    \begin{proof}
        Proof is given in appendix \ref{proof-do-calc}.
    \end{proof}
\end{theorem}
